Dynamic coherent perfect absorption in nonlinear metasurfaces

We propose a tunable coherent perfect absorber based on ultrathin nonlinear metasurfaces. The nonlinear metasurface is made of plasmonic nanoantennas coupled to an epsilon-near-zero material with a large optical nonlinearity. The coherent perfect absorption is achieved by controlling the relative phases of the input beams. We show that the optical response of the nonlinear metasurface can be tuned from a complete to a partial absorption by changing the intensity of the pump beam. The proposed nonlinear metasurface can be used to design optically tunable thermal emitters, modulators, and sensors.

==> SPIE2020.tex <==
The solution to the electromagnetic scattering off a sphere was published by Gustav Mie more than a hundred years ago. Although Ludwig Lorenz published the complete solution much earlier, the solution of the problem is widely attributed to Mie and is well-known as the Mie theory [REF1].

In Mie theory, the connection between the incident and the scattered field coefficients in the spherical basis is known as the Mie coefficient. A proper analytical model for Mie coefficients is helpful for systematic design and a better understanding of the underlying physics for phenomena in scattering theory. We look for a model that respects the physical limitations and also allows physical interpretations. To derive a model for Mie coefficients, we rely on the optical theorem enforced on optical cross sections of an isotropic particles. Using this approach, in a previous work, we have shown that for a non-absorbing particle, the following model can be used for a single Mie coefficient {a} [REF2]: a=cos(u)exp(i*u), in which {u} is an angle in the range [-π/2 π/2]. Similar forms for the model for non-absorbing particles has already been mentioned in the literature [REF3]. Please note that since for an isotropic particle, the Mie channels do not mix, the results are valid for any Mie coefficient.

A model for absorbing particles is missing. Following a similar line of arguments in the optical theorem, one can derive the following form for a Mie coefficient {a}: a=1/(1-i*tan(u)+tan(v)), where {u} (in the range [-π/2 π/2]) and {v} (in the range [0 π/2]) are the detuning and absorption Mie coefficient angles, respectively. As will be discussed in the talk, The attributed names to the angles are done after comparing the model with a Lorentzian resonance with a certain detuning, radiative and non-radiative loss. This provides physical interpretations for the attributed angles. The results are valid for any Mie coefficient of an isotropic particle, electric or magnetic, and of any order. This model can also be derived from the actual formula for the Mie coefficients of non-magnetic spheres. For a non-absorbing particle, i.e. v=0, the model can be reformulated as the model described earlier for non-absorbing particles. 

In our talk, we will show that the analytical space provided by the model is fully filled with actual electric and magnetic dipolar Mie coefficients of a sphere with varying radii and refractive index. Moreover, we will provide the conditions for critical coupling for an absorbing particle, which is v=π/4. 

A model for non-absorbing particles has already been used for systematic search of fundamental limits of optical force [REF2]. It can further be used in various fundamental studies as in metasurface capabilities. A model for absorbing particles can further facilitate the studying of absorbing systems such as perfect absorbers, torque calculations, cooling, thermal emitters etc. Using the model, one can systematically analyse through all the possible space and search for specific functions.

References:
[REF1] A. Zangwill,Modern Electrodynamics(Cambridge University Press,2013).
[REF2] Rahimzadegan, Aso, et al. "Fundamental limits of optical force and torque." Physical Review B 95.3 (2017): 035106.
[REF3] Adam, John A. "Scattering of electromagnetic plane waves in radially inhomogeneous media: ray theory, exact solutions and connections with potential scattering theory." Light Scattering Reviews 9. Springer, Berlin, Heidelberg, 2015. 101-132.
